CAD-Deform: Deformable Fitting of CAD Models to 3D Scans

Shape retrieval and alignment are a promising avenue towards turning 3D scans into lightweight CAD representations that can be used for content creation such as mobile or AR/VR gaming scenarios. Unfortunately, CAD model retrieval is limited by the availability of models in standard 3D shape collections (e.g., ShapeNet). In this work, we address this shortcoming by introducing CAD-Deform, a method which obtains more accurate CAD-to-scan fits by non-rigidly deforming retrieved CAD models. Our key contribution is a new non-rigid deformation model incorporating smooth transformations and preservation of sharp features, that simultaneously achieves very tight fits from CAD models to the 3D scan and maintains the clean, high-quality surface properties of hand-modeled CAD objects. A series of thorough experiments demonstrate that our method achieves significantly tighter scan-to-CAD fits, allowing a more accurate digital replica of the scanned real-world environment while preserving important geometric features present in synthetic CAD environments.

==> tex/0_abstract.tex <==

% LNCS guidelines indicate it should be at least 70 and at most 150 words. 
\begin{abstract}
Shape retrieval and alignment are a promising avenue towards turning 3D scans into lightweight CAD representations that can be used for content creation such as mobile or AR/VR gaming scenarios. 
Unfortunately, CAD model retrieval is limited by the availability of models in standard 3D shape collections (\eg, ShapeNet). 
In this work, we address this shortcoming by introducing CAD-Deform\footnote[1]{The code for the project: \url{https://github.com/alexeybokhovkin/CAD-Deform}}, a method which obtains more accurate CAD-to-scan fits by non-rigidly deforming retrieved CAD models. 
Our key contribution is a new non-rigid deformation model incorporating smooth transformations and preservation of sharp features, that simultaneously achieves very tight fits from CAD models to the 3D scan and maintains the clean, high-quality surface properties of hand-modeled CAD objects. 
A series of thorough experiments demonstrate that our method achieves significantly tighter scan-to-CAD fits, allowing a more accurate digital replica of the scanned real-world environment while preserving important geometric features present in synthetic CAD environments.

\keywords{scene reconstruction, mesh deformation}
\end{abstract}

==> tex/suppl_B_deformation_details.tex <==
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\cE}{\cal{E}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\bp}{\mathbf{p}}

\section{Deformation Algorithm Details}

Here we are going to provide readers with the details of mesh deformation framework implementation. In energy equation~\ref{} consider term $E_0 = \sum_{e \in \bE}\|T_e(\bV) - T_e^0\|^2_2$, where $T_e$ is $4 \times 4$ affine transformation matrix having $[0, 0, 0, 1]$ in the last row. Transformation $T_e$ can be considered as a pair $(C, \bd)$, where $C$ is $3 \times 3$ and $\bd$ is a vector of size $3$, so that the transform is $\bp = C\bp_0 + \bd$. 

==> tex/suppl_D_dame.tex <==
\section{More detailed results on local surface quality evaluation}
\label{supsec:more_dame}



